Pricing Mechanisms for Crowd-Sensed Spatial-Statistics-Based Radio Mapping

Networking on white spaces (i.e., locally unused spectrum) relies on active monitoring of spectrum usage. Spectrum databases based on empirical radio propagation models are widely adopted but shown to be error-prone, since they do not account for built environments like trees and man-made buildings. As an economically viable option, crowd-sensed radio mapping acquires more accurate local spectrum data from mobile users and constructs radio maps using spatial models such as Kriging and Gaussian Process. Success of such crowd-sensing systems presumes some incentive mechanisms to attract user participation. In this work, we consider the scenario where the platform who constructs radio environment maps makes one-time offers to selected users, and collects data from those who accept the offers. We design pricing mechanisms based on expected utility (EU) maximization, where EU captures the tradeoff between radio mapping performance (location and data quality), crowd-sensing cost and uncertainty in offer outcomes (i.e., possible expiration and rejection). Specifically, we consider sequential offering, where one best price offer is sent to the best user in each round, and batched offering, where a batch of multiple offers are made in each round. For the later, we show that EU is submodular in the discrete domain, and propose a mechanism that first fixes the pricing rule and selects users based on Unconstrained Submodular Maximization (USM); it then compares different pricing rules to find the best batch of offers in each round. We show that USM-based user selection has provable performance guarantee. Proposed mechanisms are evaluated and compared against utility-maximization-based baseline mechanisms.

==> sections/4.example_old.tex <==
\section{A Two-User Tutorial Example}\label{sec:example}
Before presenting our general model, we \rev{first present our system architecture and} provide a two-user example to illustrate the basic idea of pricing for crowd-sensed radio mapping.

\subsection{\rev{System Architecture}}\label{sec:sys_arch}
As shown in Fig.~\ref{fig:arch_pricing}, the platform acquires data periodically from users.
At the beginning of each period, the platform broadcasts a sensing task to all users in the area of interest (AoI) with specific sensing parameters (e.g., center frequency, sampling rate and FFT bin size) to ensure a consistent sensing procedure across different hardware. 
\rev{Note that the task does not specify sensing locations with twofold reasons.
First,  there is no need to do so, since the platform will take \emph{a posteriori} sampling approach to select users.
It is the relative positioning of measurements instead of exact sensing locations that matters for radio mapping. 
Second, it requires extra time and costs for users to move to target sensing locations, which means extra incentivization costs for the platform and added complexity for mechanism design\footnote{See \cite{he2014toward} for more discussions on allocation of tasks with specific locations.}}.

\begin{figure}[t]
    \centering
    \includegraphics[width = 1\columnwidth]{./figs/arch_pricing}
    \caption{\rev{Pricing-based crowd-sensing system with pricing mechanisms. 
    (1) In each period, the platform first broadcasts a sensing task to users in the area of interest.
    (2) Users who are interested and available for sensing in the current period report location and device type.
    (3) The platform determines and sends out one-time offers to selected users.
    (4) If a selected user decides to accept the offer, it performs the required sensing task. 
    All selected users will inform the platform of their decisions (and upload the data) before the deadline. 
    (5) The platform pays users who contribute data.
    }
    }
    \label{fig:arch_pricing}
\end{figure}

\rev{To avoid excessive delay due to communication delay or failure, network congestion %or no response\footnote{\rev{Users who repeatedly do not respond to offers in time will be identified and suspended by the platform.}} 
etc.,  each offer has a deadline, by which a decision has to be received by the platform (along with the data if accepted); otherwise, the offer will be expired.}

In this study, we assume no entry or other overhead costs, that is, a user does not incur a fee to communicate with the platform.
We consider users of low mobility (e.g., pedestrians), who are honest in providing their information and following the protocol. 
We assume small displacements between reported locations and eventual sensing locations. 
We will leave the high-mobility case and security considerations as future work.

\subsection{\rev{A Two-User Scenario}}
In this example, the platform wants to estimate the RSSI $Z(x_0)$ at location $x_0$.
There are two users $S=\{1,2\}$ at $x_1$ and $x_2$ in the AoI. 
In each period, each user will incur a \textit{sensing cost} $c_i > 0$ and receive an \textit{offer} $p_i > 0$, when selected by the platform.
We assume that users are \textit{rational} and will accept the offer if $c_i\leq p_i$, and reject it otherwise.
\rev{In the following discussion, we assume no expired offers and will consider them later in Section~\ref{sec:pricing_mechanism}.
}

The platform has a \textit{valuation} function $v:2^S\mapsto \mathbb{R}_+$ and a \textit{pricing} function $p:2^S\mapsto \mathbb{R}_+$.
For each set of users $A$, there is an associated \textit{value} $v(A)$ and a total price of all offers $p(A)=\sum_{i\in A}p_i$ (i.e., crowd-sensing cost for the platform), assuming that each offer is unexpired and accepted.
It makes sense for the platform, \rev{as a rational decision maker and company}, to maximize its \textit{utility} (or profit), i.e.,
\begin{equation}
\max_{A\subseteq S} u(A) = \max_{A\subseteq S} \left( v(A) - p(A) \right),
\label{eq:goal_max_utility}
\end{equation}
\rev{which is an important and widely used concept in economics (e.g., rational choice theory \cite{scott2000rational}) and measures the platform's preference over the set of users $A$.}
For convenience, we also write $v(A)$, $p(A)$ and $u(A)$ as $v_A$, $p_A$ and $u_A$, respectively.

\rev{In practice, however, the probability that an offer is accepted (and data is uploaded to the platform) by the deadline is less than 1, due to possible expiration and rejection.
Hence, only a subset of users in $A$ accept offers, and $u(A)$ is essentially the best-case utility.
In this case, it makes more senses for the platform to maximize the average-case or \textit{expected utility} (EU).
More will be discussed later in this example.}


%When $\mathcal{A}=\{i\}$ is a singleton, we also write  $p(\{i\})$ as $p_i$.
%We will next use this example to show i) how to valuate a subset of samples, and ii) how to determine which subset of users to pay at what prices from the platform's perspective.


\subsection{How to Valuate \rev{Users}}
For illustration, two RSSI data models are considered: \rev{one ignoring shadowing and noise, and the other one accounting for both}. 
\rev{Both models assume small variations in path-loss-impaired RSSIs in the AoI, and small-scale fading over small distances and time has been averaged out during sensing}.
%, since distances between users (in hundreds of meters) are usually much smaller than the distance between the AoI and the transmitter like a TV tower (in tens of kilometers). 

\subsubsection{Model I -- Shadowing-Free, Noise-Free}
This model assumes a \rev{constant but unknown RSSI} at any location within the AoI. 
When there are no measurements, both users are equally valuable, since either can provide accurate estimation.
Once one is recruited, a second user has zero marginal value.
Hence, we have $v(\{1\})$ $=v(\{2\})$ $=v({\{1,2\}})=v_0$, where $v_0$ \rev{is the value (perceived by the platform) of estimating $Z(x_0)$}.
We set $v_0=10$ for later calculations.

\subsubsection{Model II -- Shadowing-Aware, Noise-Aware}
\rev{
This model models the measured RSSI by user $i$ as a random variable,  
}
\begin{equation}
\tilde{Z}(x_i) = Z(x_i) + \epsilon_i = \mu + \delta(x_i) + \epsilon_i ~~~~ (dBm),
\end{equation}
where $\mu$ is the path-loss-impaired RSSI (unknown but constant), $\delta(x_i) \sim N(0, \sigma^2_{x_i})$ is shadowing and $\epsilon_i \sim N(0, \sigma^2_{\epsilon_i})$ is hardware noise. 
Since shadowing is a spatial phenomenon, $\{\delta(x_i)\}$ are correlated with each other and RSSIs at two closer locations are more correlated (i.e., a larger covariance), while $\{\epsilon_i\}$ are independent of each other and of shadowing.

Suppose that Ordinary Kriging\cite{cressie2015statistics} is used for RSSI estimation.
With either user, we have $\hat{Z}(x_0)=\tilde{Z}(x_i)$, where $\hat{Z}(x_0)$ is the estimated value of $Z(x_0)$. 
If both are selected, we have $\hat{Z}(x_0)=\omega_1 \tilde{Z}(x_1) + \omega_2 \tilde{Z}(x_2)$, where $\{w_i\}$ are weights\footnote{Optimal weights are obtained by minimizing the MSE.} and $\omega_1 + \omega_2=1$.
The popular metric called (minimized) mean squared error (MSE) $\mathbb{E}[(\hat{Z}(x_0)-Z(x_0))]^2$) is used to quantify the performance, and a smaller MSE implies a better estimator. 
%\vspace{0.1cm}

\rev{To translate MSE to value that is comparable to payments, the platform adopts the following valuation function,} 
\begin{equation}
v(A) = \alpha_1 \cdot \log(1 + \alpha_2 -MSE(A)) \label{eq:example_valuation_function},
\end{equation}
where $\alpha_1$, $\alpha_2$ are constants and $\alpha_2 - MSE(A)\geq 0$ for any  $A\subseteq S$. 
Since MSE is undefined for $A=\emptyset$, we set $v(\emptyset)=0$.
Intuitively, $v(\cdot)$ captures the \textit{diminishing returns} behaviors: adding a new element increases $v$ more, if there are fewer elements so far, and less, if there are more elements.
This is further formalized by the notion of \textit{submodularity}, which will be elaborated in Section~\ref{sec:submodulartiy_background}. 

We consider two cases under this model:
\begin{itemize}
\item Case 1: User 1 is closer to $x_0$ and both have the same device type.
Suppose $\sigma_{0,1}=0.5> \sigma_{0,2}=0.4$, and $\sigma^2_{\epsilon_1} = \sigma^2_{\epsilon_2}=0.2$, where $\sigma_{i,j}$ is the covariance between $\delta(x_i)$ and $\delta(x_j)$.

\item Case 2: User 1 is closer to $x_0$ but has a device that provides data of lower quality. 
Suppose $\sigma_{0,1}=0.5 > \sigma_{0,2}=0.4$ and $\sigma^2_{\epsilon_1} = 0.4 > \sigma^2_{\epsilon_2}=0.1$.
\end{itemize}
Suppose $\sigma^2_{x_i}=1$ for $i=0,1,2$ and $\sigma_{1,2}=0.3$.
Then we have $MSE(\{1\})=1.2$, $MSE(\{2\})=1.4$, and $MSE(\{1,2\})=0.84$ for Case 1, and $MSE(\{1\})=1.4$, $MSE(\{2\})=1.3$, and $MSE(\{1,2\})=0.87$ for Case 2.
As an example, we set $\alpha_1 = 10$ and $\alpha_2 = 3$. 
The value of each subset in both cases can be computed using Eq.~(\ref{eq:example_valuation_function}) and is summarized in Table~\ref{table:example_sampling_value}.

The above highlights a few things. 
First, apart from the platform's preferences (e.g., choice of valuation function and parameters like $v_0$, $\alpha_1$ and $\alpha_2$), the RSSI data model plays an important role.
Second, for a reasonable RSSI data model that considers both shadowing and noise, user locations are important (e.g., Case 1 of Model II); data quality also matters and affects valuation (e.g., Case 2 of Model II). 

\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
 & $v(\emptyset)$ & $v(\{1\})$ & $v(\{2\})$ & $v(\{1,2\})$ \\ \hline
Model I & 0 & 10 & 10 & 10 \\ \hline
Model II - Case 1 & 0 & 10.30 & 9.56 & 11.49 \\ \hline
Model II - Case 2 & 0 & 9.56 & 9.93 & 11.40 \\ \hline
\end{tabular}
\caption{Valuation of users in the two-user example. }
\label{table:example_sampling_value}
\vspace{-0.5cm}
\end{table}


\subsection{How to Select and Pay Users}\label{sec:example_how_to_select_and_pay_users}
At this point, \rev{$v(\cdot)$ is available to the platform (Table~\ref{table:example_sampling_value}}). 
The next step is to select a subset of users and determine their \rev{price offers}.
This process is called ``incentivizing''.

\subsubsection{Deterministic Cost}\label{sec:deterministic_cost} 
If \rev{user devices are treated} as specialized spectrum sensors, then sensing costs are dominated by \textit{energy (or battery)} costs \cite{pottie2000wireless}.
In this case, it is reasonable to assume \rev{deterministic sensing costs, which can be inferred from the task and device type}.
Since the platform knows $\{c_i\}$, it can set $p_{\{i\}} = c_i$ to minimize payments while guaranteeing offer acceptance,  and search for the best set of users. 

%If $\{c_i\}$ are deterministic and known to the platform, the platform can set $p_{\{i\}} = c_i$ to minimize payments and search for the best set of users.

Suppose $c_1=6$ and $c_2=5$.
Then $p_{\{1\}}=6$, $p_{\{2\}}=5$ and $p_{\{1,2\}}=p_{\{1\}} + p_{\{2\}}=11$.
The platform can afford both users under Model II, but only one under Model I. 
It is easy to see that $A^* = \{2\}$ leads to the maximum utility for both models.

\subsubsection{Random Cost with Known Distributions}\label{sec:example_known_cost_dist}
\rev{
In crowd-sensing, however, a user incurs an additional \textit{opportunity cost}, i.e., the loss of potential gain when the user decides to spend resources on sensing instead of other tasks.
It depends on the task and device status that varies over time.
%Since device status is considered as sensitive information to users, it will not be revealed to the platform due to privacy concerns.
Hence, the perceived sensing cost in each period consists of a deterministic energy cost and a random opportunity cost.

%Note the device status is considered sensitive information to users and not revealed to the platform, %it is reasonable to assume that the opportunity cost is random. 
In this case, it makes sense to model user $i$'s sensing cost as a continuous random variable $C_i$ in $[\underline{c}_i, \bar{c}_i]$, where $\bar{c}_i \geq \underline{c}_i >0$ and $\underline{c}_i$ represents the minimum energy cost.
Random variables $\{C_i\}$ are independent of each other.
Since device status is considered sensitive information, $C_i$ is private and only user $i$ knows its realization in each period, $c_i$, by evaluating the task and current device status\footnote{
\rev{In practice, we would expect a crowd-sensing application to be installed and running on users' mobile devices, which has some function that estimates the perceived sensing cost in each period based on the needed resources for the sensing task and the current device status.
%Such information is sensitive to users and thus not revealed to the platform due to privacy considerations.  
%Nevertheless, the platform can statistically estimate the cost distribution for each type of device.
Designing such a function for sensing cost estimation will be of practical importance, not only to this work, but also to many other crowd-sensing applications (e.g., \cite{koutsopoulos2013optimal}). 
But this topic is out of the scope of this paper, and will be left as future work.}
}.
We assume that the platform has only \textit{a priori} probabilistic knowledge of $C_i$.
Let $f_{C_i}(c_i)$ and $F_{C_i}(c_i)$ be the probability density function (PDF) and corresponding cumulative density function (CDF), respectively.
The PDF and $\underline{c}_i$, $\bar{c}_i$ could be learned by the platform from the empirical distribution out of prior cost declarations by users of the same device type, or from its long-term interaction with users (e.g., whether or not accept an offer with a known price).
If such prior information is absent, $C_i$ may be assumed to be uniformly distributed over $[\underline{c}_i$, $\bar{c}_i]$.
Hence, it is reasonable to assume that the platform can infer $f_{C_i}(c_i)$ or $F_{C_i}(c_i)$ based on the reported device type.

}


Since the platform does \textit{not} know $\{c_i\}$, it needs to consider possible offer rejections.
For $A=\{1\}$ or $\{2\}$, the uncertainty in user decisions implies the following utility,
\begin{equation}
u_{\{i\}} = 
\begin{cases}
    v_{\{i\}} - p_{\{i\}}, & \mbox{if user $i$ accepts the offer}\\
    0, &\mbox{otherwise}
\end{cases},
\end{equation}
which is a Bernoulli random variable and the acceptance probability is \rev{$\text{Pr}(c_i \leq p_{\{i\}}) = \int_{\underline{c}_i}^{p_{\{i\}}} f_{C_i}(c_i) dc_i = F_{C_i}(p_{\{i\}})$}.
In this case, it makes more sense to consider the EU, 
\begin{equation}
EU_{\{i\}} = \mathbb{E}[u_{\{i\}}] = (v_{\{i\}} - p_{\{i\}}) F_{C_i}(p_{\{i\}})
\label{eq:example_known_dist_max_utility_1},
\end{equation}
and the platform wants to find $p_{\{i\}}^*$ that maximizes $EU_{\{i\}}$, i.e., \textit{EU maximization}.
For $A=\{1,2\}$, the EU is given by
\begin{align}
EU_{\{1,2\}} =& (v_{\{1,2\}}-p_{\{1\}}-p_{\{2\}}) F_{C_1}(p_{\{1\}}) F_{C_2}(p_{\{2\}}) \label{eq:example_known_dist_max_utility_2} \\
&+ (v_{\{1\}}-p_{\{1\}}) F_{C_1}(p_{\{1\}}) (1-F_{C_2}(p_{\{2\}})) \nonumber \\
&+ (v_{\{2\}}-p_{\{2\}}) (1-F_{C_1}(p_{\{1\}}))F_{C_2}(p_{\{2\}}) \nonumber.
\end{align}
and the goal is to find ${\bf p}^*=[p_{\{1\}}^*,~p_{\{2\}}^*]$ that maximizes $EU_{\{1,2\}}$.
Note that in general the platform does not have to send out offers all at once and stop (i.e., \textit{single-batch} offering); it can send more batches of backup offers (i.e., \textit{multi-batch} offering) based on the knowledge of outcomes of previous offers.
For illustration, we set $C_1\sim U[4,7]$ and $C_2\sim U[5,6]$, where $U[\cdot,\cdot]$ represents the uniform distribution. 

For pricing, the platform's first thought could be setting $p_{\{i\}}=\bar{c}_i$, and the rest is the same with the deterministic-cost case. 
A natural generalization is to choose a desired probability of acceptance\footnote{Compared to choosing the same desired price for all users, it makes more sense to choose the same desired probability for all users, since users have different cost distributions in general. If all user devices are of the same type, then these two approaches are the same.} 
$\gamma \in [0,1]$ and set $p_{\{i\}}=F^{-1}_{C_i}(\gamma)$ for each user $i$, where $F^{-1}_{C_i}(\cdot)$ is the inverse CDF. 
\rev{Given $\gamma$, prices are fixed }and the platform wants to maximize the EU.
Taking Case 2 of Model II and $\gamma=0.95$ as an example, we have $p_{\{1\}} = 6.85$, $p_{\{2\}}=5.95$, $p_{\{1,2\}}=12.8$, and $A^*=\{2\}$ is the best with $EU_{\{2\}}=3.78$ by Eq.~(\ref{eq:example_known_dist_max_utility_1}) and (\ref{eq:example_known_dist_max_utility_2}).
Note that the platform may further consider user 1, if user 2 rejects the offer. 
Then the overall EU with multi-batch offering would be $EU_{\{2\}}+(1-\gamma)EU_{\{1\}} = 3.91 > EU_{\{2\}}$.

Given $A$, $\gamma$ can also be optimized in each batch. 
Taking Case 2 of Model II as an example, when $A=\{1\}$, $EU_{\{1\}} = (9.56 - (4+3\gamma))\gamma$ and $\gamma^* = 0.93$, $EU^*_{\{1\}}=2.58$.
Similarly, for $A=\{2\}$, $EU_{\{2\}}=(9.93-(5+\gamma))\gamma$ and $\gamma^*=1$, $EU^*_{\{2\}}=3.93$.
When $A=\{1,2\}$, we have $EU_{\{1,2\}}=-8.09\gamma^2+10.49\gamma$ and $\gamma^* = 0.65$, $EU_{\{1,2\}}^*=3.40$.
In this case, instead of using the same $\gamma$, the platform can also choose $\{\gamma_i\}$ for each user separately, and maximizing Eq.~(\ref{eq:example_known_dist_max_utility_2}) leads to $\gamma_1^*=0, \gamma_2^*=1$.

As we can see, the notation of utility accounts for  locations, data quality and sensing costs, and the notation of EU further considers possible offer rejections.
We can also see that user selection and \rev{price} determination are closely coupled in a pricing mechanism.
More will be discussed in Section~\ref{sec:pricing_mechanism}.

%\vspace{0.2cm}
%\noindent \textbf{Budgeted Expected Value Maximization (Eq.~\ref{eq:goal_max_value_given_budget})}\\
%\indent Similarly, the platform can maximize EV given a budget $B$ via probable-acceptance pricing with $\gamma\in(0,1]$ ($\gamma=1$ implies guaranteed-acceptance pricing) for this example.
%When $\gamma$ is close to 1, the platform can simply work with $v(\cdot)$; otherwise, it is better to work with $EV(\cdot)$ in this example, in which case $\gamma$ is optimizable.
%In all cases, we are interested in ensuring that the total payment in the worst case (i.e., no rejections) is no larger than $B$. 
%Besides, sequential and multi-batch offering can also be expected to work better than single-batch offering, and it is also possible to find optimal offers $(\mathcal{A}^*, {\bf p}^*)$ that maximizes $EV(\cdot)$ subject to ${\bf 1}^T {\bf p}\leq B$ in this example (omitted due to space limit).
%However, the optimal pricing (without first fixing prices) may not be feasible when the number of users increases. 
%More discussions are in Section~\ref{sec:value_maximization}.







==> sections/4.preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminaries}
In this section, we provide brief background on submodularity and Unconstrained Submodular Maximization (USM).

%\subsection{Background on Submodularity}
\begin{mydef}[Submodularity]\label{def:submodularity}
Let $\Omega$ be a finite set. 
A function $f: 2^\Omega \mapsto \mathbb{R}$ is submodular if for any $A,B \subseteq \Omega$, 
\begin{equation}
f(A\cup B) + f(A \cap B) \leq f(A) + f(B).
\end{equation}
\end{mydef}
Equivalently \cite{fujishige2005submodular}, a function $f$ is submodular if, for any $A \subseteq B \subseteq \Omega$ and any $i \in \Omega \setminus B$, 
\begin{equation}
f(A \cup \{i\}) - f(A) \geq f(B \cup \{i\}) - f(B).
\end{equation}
The notion of submodularity captures  \textit{diminishing returns} behaviors: adding a new element increases $f$ more, if there are fewer elements so far, and less, if there are more elements.

\begin{mydef}[(Approximately) monotonic function]
Let $\Omega$ be a finite set. 
A function $f: 2^\Omega \mapsto \mathbb{R}$ is said to be \textit{monotone} (or \textit{monotonic}), if $f(A \cup \{i\}) - f(A) \geq 0$ for any $A \subseteq \Omega$ and any $i \in \Omega\setminus A$; 
$f$ is said to be \textit{$\alpha$-approximately monotonic}, if $f(A \cup \{i\}) - f(A) \geq -\alpha$ for some small $\alpha > 0$, and for any $A\subseteq \Omega$ and any $i \in \Omega\setminus A$.
\end{mydef}

One of the most basic submodular maximization problems is USM, which is formally defined as follows.


\begin{mydef}[USM]
Given a nonnegative submodular fucntion $f:2^S \mapsto \mathbb{R}_+$,  $\max_{A \subseteq S} f(A)$ is called Unconstrained Submodular Maximization.
\end{mydef}


\begin{algorithm}
\caption{{\tt USM}}\label{algo:USM}
\LinesNumbered
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

\Input{$S$ -- ground set, $f$ -- nonnegative submodular function } 
\Output{$A_n$ (or $B_n$) -- selected subset}
$A_0 \leftarrow \emptyset$, $B_0 \leftarrow S$\;
\ForEach{$i = 1$ to $n$ }{
    $a_i \leftarrow f(A_{i-1} \cup \{u_i\}) - f(A_{i-1})$\;
    $b_i \leftarrow f(B_{i-1} \setminus \{u_i\}) - f(B_{i-1})$\;
    \lIf{$a_i\geq b_i$}{
        $A_i \leftarrow A_i \cup \{u_i\}$, $B_i \leftarrow B_{i-1}$
    }
    \lElse{
       $A_i \leftarrow A_{i-1}$,  $B_i \leftarrow B_{i-1} \setminus \{u_i\}$
    }
}

\Return $A_n$ (or equivalently $B_n$)\;
\end{algorithm}

It is well known that USM is NP-hard \cite{fujishige2005submodular, feige2011Non-Monotone} and thus heuristic-based algorithms are often used to find approximate solutions.
One state-of-art \textit{linear-time} deterministic algorithm is proposed in \cite{buchbinder2015tight} and described in Algorithm~\ref{algo:USM}, which is greedy-based and achieves a $1/3$-approximation.
That is, the algorithm obtains a solution $A$ with the guarantee that $f(A)\geq \frac{1}{3} f(OPT)$, where $OPT$ is the optimal solution.
%It takes a set $S$ and a submodular function $f(\cdot)$ as inputs, and outputs a subset $A \subseteq S$.
%As we can see, in the $i$-th iteration, it makes a greedy decision whether to add or exclude $u_i$ from its output based on marginal $f$ values $a_i$ and $b_i$, and terminates when all elements in $S$ are touched once.
%Hence, its complexity is $\mathcal{O}(n)$ in terms of the number of evaluating $f$.
%It achieves an performance guarantee of $1/3$. 


%\begin{mylemma}{(\hspace{.01cm}\cite{buchbinder2015tight})}\label{lemma:USM_bound}
%Given a nonnegative submodular function $f:2^S \mapsto \mathbb{R}_+$, Algorithm~\ref{algo:USM} obtains a solution $A$ with a $1/3$ approximation for USM, that is, $f(A)\geq \frac{1}{3} f(OPT)$, where $OPT$ is the optimal solution.
%\end{mylemma}

==> sections/7.evaluation.1st.round.tex <==
\section{Evaluation}\label{sec:evaluation}
In this section, \rev{we first study the impact of $\gamma$ on USM-u and USM-EU based batched offering for two type of cost distributions, i.e., uniform and truncated normal distributions.
Then we compare the performance of sequential offering and batched offering with PA pricing.
Finally, we study the impact of $P_d$ on proposed schemes. 
}
%we first present our simulation setup. 
%Then we evaluate the performance of single-batch PA pricing and study the relationship between achieved EU and the choice of $\gamma$ for two types of cost distributions, that is, uniform and truncated normal distributions.
%We further compare the performance of single-/multi-batch PA pricing against sequential optimal pricing.

For convenience, we refer to USM-based user selection  with the best-case utility $u_\gamma(\cdot)$ in batched offering as USM-u, and that with the (approximated) expected/average-case utility $\hat{EU}_\gamma(\cdot)$ as USM-EU.

\subsection{Simulation Setup}
We generate random user locations from the spatial Poisson process. 
Fig.~\ref{fig:60_users_poisson_topo} is a sample topology of 60 users over a 6km-by-6km region\footnote{For a wide AoI, the platform may divide it into smaller AoIs, each of which has a reasonable amount of users.
Doing so can leverage the nature of spatial interpolation techniques (e.g., local estimator) and may potentially improve radio mapping.
Besides, it can effectively reduce computing costs. 
}, which is discretized into a total of 169 points with a resolution of 450 meters. 
The closest two users are 120 meters apart.
We assume an exponential kernel function $\mathcal{K}(d) = 15.5\cdot \exp(-\frac{d}{0.7})$, as shown in Fig.~\ref{fig:cov_func}.
It is adapted from the fitted variogram based on real measurements in \cite{Ying2015-ju}. 
Given the above settings, we do not observe negative marginal MI values and thus we set $\epsilon=0$.
% and it is reasonable to believe $MI(\cdot)$ is monotone non-decreasing. 

\begin{figure}[ht]
        \centering
        \begin{subfigure}[b]{0.49\columnwidth}
                \includegraphics[width=1\textwidth]{figs/simulation/60_users_poisson_topo}
                \caption{Sample topology}
                \label{fig:60_users_poisson_topo}
        \end{subfigure}
        \begin{subfigure}[b]{0.49\columnwidth}
                \includegraphics[width=1\textwidth]{figs/cov_func}
                \caption{Kernel function}
                \label{fig:cov_func}
        \end{subfigure}
        \caption{(a) Sample topology of 60 users (in red) in a 6km-by-6km area that is discretized into a mesh grid of 169 points (in blue). (b) The kernel function $\mathcal{K}(d) = 15.5\cdot \exp(-\frac{d}{0.7})$.}
        \label{fig:simu_topology_and_cov_func}
\end{figure}


\begin{figure}[ht]
        \centering
        \begin{subfigure}[b]{0.49\columnwidth}
                \includegraphics[width=1\textwidth]{figs/simulation/cost_dist_pdf}
                \caption{}
                \label{fig:simulation_cost_dist_pdf}
        \end{subfigure}
        \begin{subfigure}[b]{0.49\columnwidth}
                \includegraphics[width=1\textwidth]{figs/simulation/cost_dist_cdf}
                \caption{}
                \label{fig:simulation_cost_dist_cdf}
        \end{subfigure}
        \caption{(a) PDF and (b) CDF of UN and TN distributions.}
        \label{fig:simulation_cost_dist}
\end{figure}

We assume that the range of user $i$'s sensing cost is $[\underline{c}_i, \underline{c}_i + \Delta c]$, where $\Delta c > 0$ and $\underline{c}_i$ values are randomly generated from a uniform distribution $U[0.1, 0.2]$.
As shown in Fig.~\ref{fig:simulation_cost_dist}, two types of cost distributions are considered: (1) uniform (UN) and (2) truncated normal (TN) distributions.
Here TN is the normal distribution 
$N(\underline{c}_i, (\Delta c/3)^2)$ truncated to $[\underline{c}_i, \underline{c}_i + \Delta c]$.
Compared to UN, TN represents the case where the majority of users have sensing costs closer to energy costs.
Besides, we use the same set of noise variances independently drawn from $U[0.5,1]$ throughout our simulation.

\subsection{Baseline Mechanisms Based on Utility Maximization}

\subsection{Impact of Number of Iterations on $\hat{EU}(\cdot)$}

\subsection{USM-u vs. USM-EU in Single-Batch Offering}
In this experiment, we compare the performance of USM-u and USM-EU in singe-batch offering with PA pricing. 
We randomly selected 30 or 60 users and approximated $EU_{\gamma}(\cdot)$ by averaging over 50 iterations of MC simulations.
We set $\kappa$ in $v(\cdot)$ (Eq.~(\ref{eq:valuation_function})) to 4 or 8, and $\Delta c$ to 0.1 or 0.5.  
\rev{We set $P_d=1$, i.e., an offer is either accepted or rejected, and none is expired.} 
A total of 30 iterations were conducted, and a different seed was used for generating users and cost distributions in each iteration.
But in the $i$-th iteration, the same set of users and cost distributions were used across different $\gamma$ values for fair comparison.
Average results are provided in Fig.~\ref{fig:USM_u_vs_USM_EU_avg}.

%\begin{figure}[ht]
%\centering
%\begin{subfigure}[b]{0.49\columnwidth}
%        \includegraphics[width=1\textwidth]{figs/USM_u_vs_USM_EU/PA_pricing_30_users_kappa_8_sample_uniform}
%        \caption{UN cost distribution}
%        \label{fig:PA_pricing_30_users_kappa_8_sample_uniform}
%\end{subfigure}
%\begin{subfigure}[b]{0.49\columnwidth}
%        \includegraphics[width=1\textwidth]{figs/USM_u_vs_USM_EU/PA_pricing_30_users_kappa_8_sample_truncated_normal}
%        \caption{TN cost distribution}
%        \label{fig:PA_pricing_30_users_kappa_8_sample_truncated_normal}
%\end{subfigure}
%\caption{USM-u vs. USM-EU for (a) UN and (b) TN  distributions in a typical iteration for $n=30$, $\kappa=8$ and $\Delta c = 0.5$.
%$\mathcal{A}_{u}$ and $\mathcal{A}_{EU}$ are the obtained solutions by USM-u and USM-EU.
%$\hat{EU}(\mathcal{A}_{u})$ and $\hat{EU}(\mathcal{A}_{EU})$ are approximated EU values, whose lower bounds are $\gamma u_\gamma(A_{u})$ and $\gamma u_\gamma(\mathcal{A}_{EU})$, respectively.}
%\label{fig:USM_u_vs_USM_EU_one_iteration}
%\end{figure}



\begin{figure}[h!]
        \centering
        \begin{subfigure}[b]{0.49\columnwidth}
                \includegraphics[width=1\textwidth]{figs/USM_u_vs_USM_EU/avg_30_users_kappa_8_delta_0_5}
                \caption{$n=30$, $\kappa=8$, $\Delta c = 0.5$}
                \label{fig:avg_30_users_kappa_8_delta_0_5}
        \end{subfigure}
        \begin{subfigure}[b]{0.49\columnwidth}
                \includegraphics[width=1\textwidth]{figs/USM_u_vs_USM_EU/avg_60_users_kappa_8_delta_0_5}
                \caption{$\boldsymbol{n=60}$, $\kappa=8$, $\Delta c = 0.5$}
                \label{fig:avg_60_users_kappa_8_delta_0_5}
        \end{subfigure}
        \begin{subfigure}[b]{0.49\columnwidth}
                \includegraphics[width=1\textwidth]{figs/USM_u_vs_USM_EU/avg_30_users_kappa_8_delta_0_1}
                \caption{$n=30$, $\kappa=8$, $\boldsymbol{\Delta c = 0.1}$}
                \label{fig:avg_30_users_kappa_8_delta_0_1}
        \end{subfigure}
        \begin{subfigure}[b]{0.49\columnwidth}
                \includegraphics[width=1\textwidth]{figs/USM_u_vs_USM_EU/avg_30_users_kappa_4_delta_0_5}
                \caption{$n=30$, $\boldsymbol{\kappa=4}$, $\Delta c = 0.5$}
                \label{fig:avg_30_users_kappa_4_delta_0_5}
        \end{subfigure}
        \caption{Average performance of USM-u and USM-EU in terms of (approximated) EU for UN and TN cost distributions under different settings. We set $P_d=1$.}
        \label{fig:USM_u_vs_USM_EU_avg}
\end{figure}

%Fig.~\ref{fig:USM_u_vs_USM_EU_one_iteration} illustrates the comparison between USM-u and USM-EU in a single iteration.
%We first notice that the lower bound $\gamma u(\mathcal{A})$ is reasonably tight when $\gamma\geq 0.9$, but loose for smaller $\gamma$. 
%We can also see that the performance of both USM-u and USM-EU depends on the choice of $\gamma$, which suggests the possibility of optimizing USM-u and USM-EU over $\gamma$.

In Fig.~\ref{fig:avg_30_users_kappa_8_delta_0_5}, we observe that $\gamma^*$ is less than 1 for both USM-u and USM-EU under both UN and TN distributions. 
This is mainly because with a smaller $\gamma$, the platform can save money per user and send out more offers.
Although each offer is less likely to be accepted, the platform can still benefit from it and achieve a greater EU.  
Besides, the fact that the platform can save more per user under TN than UN with the same $\gamma$ explains why it can obtain a higher EU with the same scheme under TN than UN. 
Similar behaviors are observed in Fig.~\ref{fig:avg_60_users_kappa_8_delta_0_5} and \ref{fig:avg_30_users_kappa_4_delta_0_5}.
But in Fig.~\ref{fig:avg_30_users_kappa_8_delta_0_1} when $\Delta c$ is changed from $0.5$ to $0.1$, the uncertainty in opportunity costs is reduced and energy costs become more dominant. 
In this case, the platform will not save much per user with a small $\gamma$ and should choose a larger $\gamma$.

Furthermore, as shown in Fig.~\ref{fig:avg_30_users_kappa_8_delta_0_5}, USM-EU is slightly better than USM-u with $\gamma$ between 0.3 and 0.6 under UN, but their performance is very close for $\gamma\leq 0.2$ under UN and for all $\gamma$ values under TN. 
This is mainly because in those cases, both schemes will send out offers to more or all users (30 max. in this setting) and thus achieve very close EU.
When there are more users (Fig.~\ref{fig:avg_60_users_kappa_8_delta_0_5}), we again observe the advantage of USM-EU over USM-u under both UN and TN.
With less uncertainty in sensing costs (Fig.~\ref{fig:avg_30_users_kappa_8_delta_0_1}), USM-EU is less advantageous. 
In Fig.~\ref{fig:avg_30_users_kappa_4_delta_0_5}, when $\kappa$ is small, each user is less valuable and USM-u selects fewer users, since it assumes no \rev{expired or rejected offers}.
In contrast, USM-EU considers the average-case utility and is more aggressive in user selection, which explains its better performance than USM-u with the same small $\gamma$. 

\subsection{Batched Offering vs. Sequential Offering}\label{sec:UM_PA_vs_OP}
In this simulation, we compare the following schemes: 
\rev{
\begin{itemize}
\item SB-u/EU: single-batch offering with USM-u or USM-EU;
\item MB-u/EU: multi-batch offering with USM-u or USM-EU;
\item SE: sequential offering.
\end{itemize}
}

\begin{figure}[ht]
\centering
\begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=1\textwidth]{figs/BA_vs_SE/impact_num_of_users_uniform}
        \caption{}
        \label{fig:impact_num_of_users_uniform}
\end{subfigure}
\begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=1\textwidth]{figs/BA_vs_SE/impact_num_of_users_truncated_normal}
        \caption{}
        \label{fig:impact_num_of_users_truncated_normal}
\end{subfigure}
\caption{Comparison of SB-u, MB-u, SB-EU, MB-EU and SE with different numbers of users under (a) UN and (b) TN cost distributions.}
\label{fig:PA_vs_OP_num_of_users}
\end{figure}

We randomly selected $n$ out of 60 users, and generated a set of noise variances and cost distributions, which were used in all iterations for each $n$. 
In the $i$-th iteration, we generated a different set of sensing costs from users' cost distributions independently, and used them across different schemes for fair comparison.
We set $\Delta c = 0.5$, and varied $n$ or $\kappa$ to study their impacts on the average utility achieved by the platform.
We set $P_d=1$.
All results are averaged over 30 iterations. 

We first fixed $\kappa=2$ and varied $n$ from 10 to 60.
As shown in Fig.~\ref{fig:PA_vs_OP_num_of_users}, all schemes work better as $n$ increases. 
For both UN and TN, multi-batch offering is always better than single-batch offering, and such advantage is greater for USM-u than USM-EU. 
For instance, MB-u is $30.7\%$ and $14.6\%$ better than SB-u on average for UN and TN, respectively, while MB-EU is only $5.0\%$ and $2.6\%$ better than SB-EU on average.
This is again because USM-u is conservative in determining the first batch, and more batches can effectively improve the achieved utility.
In contrast, USM-EU is generous in the first batch, which makes following batches less beneficial.
In all schemes, $\gamma^*$ in each batch decreases as the platform sends out more batches. 

Interestingly, although SB-u is much worse than SB-EU, MB-u achieves close performance with MB-EU.
Specifically, SB-EU is $31.3\%$ and $16.2\%$ better than SB-u, but MB-u is only $5.1\%$ and $3.6\%$ worse than MB-EU on average for UN and TN, respectively. 
The fact that USM-u is more computationally efficient makes MB-u a good choice in practice. 
Besides, we observe that SE performs the worst, since it always makes a local decision without optimizing the utility in a global sense.
%Besides, it tends to offer overly high prices to first few users, and much lower prices to following users, resulting in few acceptances.


\begin{figure}[ht]
\centering
\begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=1\textwidth]{figs/PA_vs_OP/impact_kappa_uniform}
        \caption{}
        \label{fig:impact_kappa_uniform}
\end{subfigure}
\begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=1\textwidth]{figs/PA_vs_OP/impact_kappa_truncated_normal}
        \caption{}
        \label{fig:impact_kappa_truncated_normal}
\end{subfigure}
\caption{Comparison of SB-u, MB-u, SB-EU, MB-EU and SE with different $\kappa$ values for (a) UN and (b) TN cost distributions.
Note that MB-u, SB-EU and MB-EU are almost indistinguishable in (b), but MB-EU always performs the best.}
\label{fig:PA_vs_OP_kappa}
\end{figure}

We then fixed $n=60$ and varied $\kappa$ from 1 to 6.
As shown in Fig.~\ref{fig:PA_vs_OP_kappa}, the averaged utility obtained by each scheme increases as $\kappa$ increases, because the platform values each unit of MI (log-scaled) more and is also able to recruit more users.
Besides, multi-batch offering is better than single-batch offering, as expected.
Furthermore, the gap between MB-EU and MB-u is becoming smaller when $\kappa$ increases.
For UN, MB-EU is $21.4\%$ better than MB-u with $\kappa=1$ but only $1.6\%$ better with $\kappa=6$.
The corresponding numbers are $16.6\%$ and $1.0\%$ for TN. 
This is because a larger $\kappa$ allows the platform to recruit more users, and the average utility tends to be saturated due to its diminishing returns property. 
Furthermore, batched offering schemes again perform better than SE.

To summarize, multi-batch offering is always better than single-batch offering, and the improvement is more significant for USM-u than USM-EU.
Although SB-u performs worse than SB-EU, MB-u achieves close performance with MB-EU in many cases. 
Considering USM-u is more computationally efficient, we believe that MB-u is a better choice in practice. 

\subsection{Impact of $P_d$}
\TODO{One more experiment}

\begin{figure}[ht]
\centering
\begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=1\textwidth]{figs/BA_vs_SE/impact_num_of_users_uniform}
        \caption{}
        \label{fig:impact_of_P_d_uniform}
\end{subfigure}
\begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=1\textwidth]{figs/BA_vs_SE/impact_num_of_users_truncated_normal}
        \caption{}
        \label{fig:impact_of_P_d_truncated_normal}
\end{subfigure}
\caption{Comparison of SB-u, MB-u, SB-EU, MB-EU and SE with different numbers of users under (a) UN and (b) TN cost distributions.}
\label{fig:impact_of_P_d}
\end{figure}


%\begin{figure}[ht]
%\centering
%\begin{subfigure}[b]{0.49\columnwidth}
%        \includegraphics[width=1\textwidth]{figs/PA_vs_OP/impact_kappa_uniform_incomplete}
%        \caption{}
%        \label{impact_kappa_uniform_incomplete}
%\end{subfigure}
%\begin{subfigure}[b]{0.49\columnwidth}
%        \includegraphics[width=1\textwidth]{figs/PA_vs_OP/impact_kappa_truncated_normal_incomplete}
%        \caption{}
%        \label{impact_kappa_truncated_normal_incomplete}
%\end{subfigure}
%\caption{Comparison of PA-SB, PA-MB and OP-SE with different $\kappa$ values for (a) uniform and (b) truncated normal cost distributions. \hl{(incomplete)}}
%\label{fig:PA_vs_OP_kappa}
%\end{figure}

%
%\subsection{Pricing Mechanisms for Budgeted VM}
%\subsubsection{PA Pricing with Single-Batch Offering}
%In this simulation, we compare the performance of GS-v and GS-EV in terms of EV for different $\gamma$ values. 
%Both want to maximize $EV_{\gamma}(\cdot)$ via the GS algorithm.
%But GS-v searches for the set that maximizes $v_{\gamma}(\cdot)$ hoping that it may result in a reasonably good EV, while GS-EV aims to maximize MC-approximated $EV_{\gamma}(\cdot)$ directly.
%
%We used a similar setting as in UM simulations: 30 randomly selected or all users out of 60 users, and $EV_{\gamma}$ is obtained by averaging over 50 MC iterations. 
%The $\kappa$ value does not affect the GS algorithm, we set it to 1. 
%We set $\Delta c$ to 0.1 or 0.5, and $B$ to 3 or 6. 
%Results are averaged over 30 iterations. 
%
%\begin{figure}[ht]
%\centering
%\begin{subfigure}[b]{0.49\columnwidth}
%        \includegraphics[width=1\textwidth]{figs/VM_GSv_vs_GSEV/one_instance_uniform}
%        \caption{UN cost distribution}
%        \label{fig:VM_PA_one_instance_uniform}
%\end{subfigure}
%\begin{subfigure}[b]{0.49\columnwidth}
%        \includegraphics[width=1\textwidth]{figs/VM_GSv_vs_GSEV/one_instance_truncated_normal}
%        \caption{TN cost distribution}
%        \label{fig:VM_PA_one_instance_truncated_normal}
%\end{subfigure}
%\caption{GS-v versus GS-EV for (a) uniform and (b) truncated normal cost distributions in one iteration. In this simulation, $n=30$, $B=3$ and $\Delta c = 0.5$.
%$\mathcal{A}_{v}$ and $\mathcal{A}_{EV}$ are the obtained solution sets by GS-v and GS-EV, respectively.
%$\hat{EV}(\mathcal{A}_{v})$ and $\hat{EV}(\mathcal{A}_{EV})$ are approximated EV values, and the corresponding lower bounds are $\gamma v(A_{v})$ and $\gamma v(\mathcal{A}_{EV})$.}
%\label{fig:VM_PA_one_instance}
%\end{figure}
%
%Fig.~\ref{fig:VM_PA_one_instance} shows the comparison between GS-v and GS-EV in one iteration. 
%We again see that the lower bound is reasonable for $\gamma \geq 0.9$, but not any more for small values.
%Besides, we observe that GS-v and GS-EV have very close performance. 
%For both distributions, EV increases in general as $\gamma$ increases, and the maximum is reached when $\gamma=0.9$ (more obvious for truncated normal distributions).
%The above again indicates that EV can be optimized via $\gamma$. 
%
%The averaged results are provided in Fig.~\ref{fig:VM_GSv_vs_GSEV}.
%Under all settings, GA pricing often maximizes EV for UN distributions, but PA pricing is more advantageous for TN distributions due to similar reasons as explained in VM simulations: a smaller $\gamma$ saves more per user and allows more users to be recruited for TN distributions.  
%By cross-comparing the results, we may observe that increasing $n$ or $B$ leads to an increase in EV, and reducing the cost fluctuation weakens the advantage of PA pricing. 
%
%\begin{figure}[h!]
%        \centering
%        \begin{subfigure}[b]{0.49\columnwidth}
%                \includegraphics[width=1\textwidth]{figs/VM_GSv_vs_GSEV/avg_30_users_B_3_delta_0_5}
%                \caption{$n=30$, $B=3$, $\Delta c = 0.5$}
%                \label{fig:avg_30_users_B_3_delta_0_5}
%        \end{subfigure}
%        \begin{subfigure}[b]{0.49\columnwidth}
%                \includegraphics[width=1\textwidth]{figs/VM_GSv_vs_GSEV/avg_60_users_B_3_delta_0_5}
%                \caption{$\boldsymbol{n=60}$, $B=3$, $\Delta c = 0.5$}
%                \label{fig:avg_60_users_B_3_delta_0_5}
%        \end{subfigure}
%        \begin{subfigure}[b]{0.49\columnwidth}
%                \includegraphics[width=1\textwidth]{figs/VM_GSv_vs_GSEV/avg_30_users_B_3_delta_0_1}
%                \caption{$n=30$, $B=3$, $\boldsymbol{\Delta c = 0.1}$}
%                \label{fig:avg_30_users_B_3_delta_0_1}
%        \end{subfigure}
%        \begin{subfigure}[b]{0.49\columnwidth}
%                \includegraphics[width=1\textwidth]{figs/VM_GSv_vs_GSEV/avg_30_users_B_6_delta_0_5}
%                \caption{$n=30$, $\boldsymbol{B=6}$, $\Delta c = 0.5$}
%                \label{fig:avg_30_users_B_6_delta_0_5}
%        \end{subfigure}
%        \caption{Average performance of GS-v and GS-EV in terms of EV for uniform (U) and truncated normal (TN) cost distributions under different settings. Results are averaged over 30 iterations.}
%        \label{fig:VM_GSv_vs_GSEV}
%\end{figure}
%
%\subsubsection{Single-Batch versus Multi-Batch Offering}
%In this simulation, we are interested in comparing:
%\begin{itemize}
%\item PA-SB-v/EV: PA-based single-batch offering with GS-v/GS-EV;
%\item PA-MB-v/EV: PA-based multi-batch offering with GS-v/GS-EV.
%\end{itemize}
%
%We used similar settings as in Section~\ref{sec:UM_PA_vs_OP}, where $n$ users are randomly selected out of 60 users, $\Delta c=0.5$ and all results are averaged over 30 iterations.
%We first fixed $B=3$ and varied $n$ from 10 to 60 with an increment of 10.
%As shown in Fig.~\ref{fig:VM_SB_vs_MB_impact_of_n}, values achieved by all schemes tend to increase when $n$ increases and then hit the plateau after some point. 
%As expected, PA-MB performs better than PA-SB for both GS-v and GS-EV, since it sends backup offers in the case of rejections of previous offers.
%But such improvement is small, since both prefer offering prices with large $\gamma$ values (e.g., $\gamma \geq 0.8$), and thus only one batch is sent most of the time. 
%For both distributions, GS-EV has very close performance with GS-v, because a user preferred by GS-v is also more valuable than others (given the same $\gamma$) and is very likely to be selected by GS-EV.
%
%We then fixed $n$ to 60 and varied $B$ from 1 to 6, and the averaged results are provided in Fig.~\ref{fig:VM_SB_vs_MB_impact_of_B}.
%When $B$ increases, the platform can recruit more users and achieve a higher total value, but the marginal gain of one additional unit of $B$ is diminishing and will eventually become zero, since $n$ is fixed. 
%PA-MB performs slightly better than PA-SB for truncated normal cost distributions, and GS-EV and GS-v again have very close performance, as explained previously. 
%
%
%\begin{figure}[ht]
%\centering
%\begin{subfigure}[b]{0.49\columnwidth}
%        \includegraphics[width=1\textwidth]{figs/VM_SB_vs_MB/impact_num_of_users_uniform}
%        \caption{}
%        \label{fig:VM_SB_vs_MB_impact_num_of_users_uniform}
%\end{subfigure}
%\begin{subfigure}[b]{0.49\columnwidth}
%        \includegraphics[width=1\textwidth]{figs/VM_SB_vs_MB/impact_num_of_users_truncated_normal}
%        \caption{}
%        \label{fig:VM_SB_vs_MB_impact_num_of_users_truncated_normal}
%\end{subfigure}
%\caption{Comparison of PA-SB-v, PA-MB-v, PA-SB-EV and PA-MB-EV for different number of users for (a) uniform and (b) truncated normal cost distributions.}
%\label{fig:VM_SB_vs_MB_impact_of_n}
%\end{figure}
%
%\begin{figure}[ht]
%\centering
%\begin{subfigure}[b]{0.49\columnwidth}
%        \includegraphics[width=1\textwidth]{figs/VM_SB_vs_MB/impact_budget_uniform}
%        \caption{}
%        \label{fig:VM_SB_vs_MB_impact_B_uniform}
%\end{subfigure}
%\begin{subfigure}[b]{0.49\columnwidth}
%        \includegraphics[width=1\textwidth]{figs/VM_SB_vs_MB/impact_budget_truncated_normal}
%        \caption{}
%        \label{fig:VM_SB_vs_MB_impact_B_truncated_normal}
%\end{subfigure}
%\caption{Comparison of PA-SB-v, PA-MB-v, PA-SB-EV and PA-MB-EV for different budgets for (a) uniform and (b) truncated normal cost distributions.}
%\label{fig:VM_SB_vs_MB_impact_of_B}
%\end{figure}
%


==> sections/archive/spatial_model_old.tex <==
\section{Our RSSI and Valuation Model}\label{sec:spatial_model}
In REM, we are not only interested in RSSIs at measured user locations, but also those at unmeasured locations with (possible) user presence. 
Although linear regression like Kriging \cite{Cressie1991-ac} as explained in Section~\ref{sec:example} often gives excellent predictions, it does not provide a measure of prediction uncertainty, while a \textit{Gaussian process} (GP) naturally generalizes linear regression, which quantifies uncertainty about predictions. 

In this work, we will work with the noise-aware RSSI model (i.e., Model II in Section~\ref{sec:example}) and define a metric based on \textit{mutual information} (MI) to measure sampling performance, as well as the platform's valuation function to translate MI to sampling values. 
We further explore interesting structural properties like \textit{submodulaity} with the valuation function.


\subsection{Spatial RSSI Model}
In general, the front-end RSSI at location $x \in \mathbb{R}^2$ with AoI is
\begin{equation}
Z(x) = \mu(x) + \delta(x)
\end{equation}
where $\mu(x)$ is the path-loss-impaired RSSI (in dBm), and $\delta(x)\sim N(0, \sigma_x^2)$ represents shadowing (Gaussian in the dB scale). 
The user $i$' device introduces additive hardware noise and the eventual noisy sample $Z_i(x_i)$ is given by
\begin{equation}
Z_i(x_i) = Z(x_i) + \epsilon_i
\end{equation}
and $\epsilon_i \sim N(0, \sigma^2_i)$ only depends on its device type and is independent of locations and other devices.
Hence, $Z_i(x_i) \sim N(\mu_{x_i}, \sigma^2_{x_i} + \sigma^2_{\epsilon_i})$.
For simplicity, we write $Z(x_i)$ as $Z_i$ and $Z_i(x_i)$ as $\tilde{Z}_i$, where ``\textapprox'' is used to stress the presence of noise.

In GP model, the set of $m$ noisy samples at locations $\mathcal{A}$ constitutes a Gaussian random vector $\tilde{Z}_\mathcal{A}=[\tilde{Z}_1,...,\tilde{Z}_m]$ with a joint distribution of 
\begin{equation}
f_{\tilde{Z}_\mathcal{A}}(\tilde{z}_{\mathcal{A}}) = \frac{1}{(2\pi)^{n/2} |\Sigma_{\tilde{\mathcal{A}}\tilde{\mathcal{A}}}|} e^{-\frac{1}{2} (\tilde{z}_{\mathcal{A}} - \mu_{\mathcal{A}})^T \Sigma^{-1}_{\tilde{\mathcal{A}} \tilde{\mathcal{A}}} (\tilde{z}_{\mathcal{A}} - \mu_{\mathcal{A}}) }
\end{equation}
where $\tilde{z}_\mathcal{A}=[\tilde{z}_1,...,\tilde{z}_m]$ is a realization of $\tilde{Z}_\mathcal{A}$, $\mu_\mathcal{A}=[\mu_{x_1},...,\mu_{x_m}]$  the mean vector and $\Sigma_{\tilde{\mathcal{A}}\tilde{\mathcal{A}}}$ the covariance matrix with the $(i,j)$-th entry being $\text{Cov}(\tilde{Z}_i,\tilde{Z}_j)$. 
Since $\{\epsilon_i\}$ are zero-mean and independent of $\{Z_i\}$, we have $\text{Cov}(\tilde{Z}_i,\tilde{Z}_i)=\text{Cov}(Z_i,Z_i) + \sigma_i^2$, and $\text{Cov}(\tilde{Z}_i,\tilde{Z}_j) = \text{Cov}(Z_i,Z_j)$ for $i\neq j$, which captures the spatial correlation in shadowing. 
Note that every finite subset of $\tilde{Z}_\mathcal{A}$ is jointly Gaussian.

Estimating $\Sigma$ can be difficult, and it is typically assumed that the covariance is a function of distance, that is, $\text{Cov}(Z_i, Z_j) = \mathcal{K}(||x_i - x_j||)$, where $\mathcal{K}(\cdot)$ is the kernel or covariance function\footnote{In this study, we assume $\mathcal{K}(\cdot)$ is both stationary (i.e., a function of location displacement) and isotropic (i.e., a function of distance)\cite{Krause2008-zh}. However, our following discussions are applicable to general kernel functions.}.  
Conditioned on a set of noisy measurements $\tilde{{\bf z}}_{\mathcal{A}}$, the front-end RSSI $Z_y$ at an unmeasured location $y$ is a Gaussian with a conditional mean $\mu_{y|\tilde{\mathcal{A}}}$ and variance $\sigma^2_{y|\tilde{\mathcal{A}}}$,
\begin{align}  \label{eq:cond_mean}
\mu_{y|\tilde{\mathcal{A}}} &= \mu_y + \Sigma_{y \tilde{\mathcal{A}}} \Sigma^{-1}_{\tilde{\mathcal{A}}\tilde{\mathcal{A}}} (\tilde{{\bf x}}_{\mathcal{A}} - \mu_{\mathcal{A}}) \\ \nonumber
&= \mu_y + \Sigma_{y \mathcal{A}} \left(\Sigma_{\mathcal{A}\mathcal{A}} + D_{\tilde{\mathcal{A}}} \right)^{-1} (\tilde{{\bf x}}_{\mathcal{A}} - \mu_{\mathcal{A}}) \\
\sigma^2_{y |\tilde{\mathcal{A}}} &= \sigma^2_y - \Sigma_{y \tilde{\mathcal{A}}} \Sigma^{-1}_{\tilde{\mathcal{A}}\tilde{\mathcal{A}}}\Sigma_{\tilde{\mathcal{A}}y}  \label{eq:cond_var}\\ \nonumber
&= \sigma^2_y - \Sigma_{y \mathcal{A}} \left(\Sigma_{\mathcal{A}\mathcal{A}} + D_{\tilde{\mathcal{A}}}\right)^{-1}\Sigma_{\mathcal{A}y}
\end{align}
where $\Sigma_{y \mathcal{A}}$ is the covariance vector with each entry for each $i\in \mathcal{A}$ which has a value of $\mathcal{K}(||y-x_i||)$, and $D_{\tilde{\mathcal{A}}}$ is an $m$-by-$m$ diagonal matrix with $d_i = \sigma^2_{\epsilon_i}$. 
Note that computing predictive distributions with Eq.~\ref{eq:cond_mean} and \ref{eq:cond_var} requires the mean and covariance functions to be known, which can usually be estimated from previous measurements\footnote{In \cite{Phillips2012-uq}, authors demonstrated how to use a predictive (empirical) path loss model to estimate the mean process $\mu{x}$. This procedure is called \textit{detrending}. In the same paper as well as \cite{Ying2015-ju}, authors have shown how to estimate an empirical semivarigram $\gamma(\cdot)$ (which is assumed to be isotropic and stationary) and fit it with parametric models. The relationship between $\gamma(\cdot)$ and $\mathcal{K}(\cdot)$ is $\mathcal{K}(d_{ij})=\mathcal{K}(0)-\gamma(d_{ij})$, where $d_{ij}=||s_i-s_j||$. }. 

\subsection{Sampling Design}
Denote the set of user locations as $\mathcal{S}$, and the set of possible user presence (e.g., a grid discretization of an AoI) as $\mathcal{U}$. 
Denote the entire set of locations of interest as $\mathcal{V}=\mathcal{S}\cup\mathcal{U}$. 
The goal of sampling is to choose the best set of noisy samples $\{\tilde{Z}_i: i\in \mathcal{A}\}$, where $\mathcal{A}\subseteq \mathcal{S} \subseteq \mathcal{V}$, to predict front-end RSSI values at all locations $\{Z_i: i \in \mathcal{V}\}$.
Note that $\tilde{Z}_i\neq Z_i$ for $i\in \mathcal{A}$ due to the presence of noise. 
The above optimization is called \textit{sampling design} in spatial statistics.

We define $MI: 2^\mathcal{S}\mapsto \mathbb{R}_+$ to quantify the reduction of uncertainty about the front-end RSSI estimates at all locations given selected sample locations,
\begin{equation}\label{eq:MI_definition}
MI(\mathcal{A}) = I(Z_{\mathcal{V}}; \tilde{Z}_{\mathcal{A}}) = H(Z_{\mathcal{V}}) - H(Z_{\mathcal{V}} | \tilde{Z}_{\mathcal{A}})
\end{equation}
where $H(Z_{\mathcal{V}} | \tilde{Z}_{\mathcal{A}})$ is the conditional entropy that captures prediction uncertainty in $Z_{\mathcal{V}}$ given $\tilde{Z}_\mathcal{A}$. 

Since $\tilde{Z}_\mathcal{A} = Z_\mathcal{A} + \epsilon_\mathcal{A}$, and $\{\epsilon_i: i \in \mathcal{A}\}$ are independent of each other as well as all variables in $Z_\mathcal{V}$, it means the variables in $\tilde{Z}_\mathcal{A}$ are independent given $Z_\mathcal{A}$ or $Z_\mathcal{V}$.
Then we have
\begin{align}
H(Z_\mathcal{V}|\tilde{Z}_{\mathcal{A}}) &= H(Z_\mathcal{V}\cup\tilde{Z}_{\mathcal{A}}) - H(\tilde{Z}_\mathcal{A}) \nonumber \\
&= H(\tilde{Z}_\mathcal{A}|Z_\mathcal{V}) + H(Z_\mathcal{V}) - H(\tilde{Z}_\mathcal{A}) \nonumber \\
&= H(Z_\mathcal{V}) - H(\tilde{Z}_\mathcal{A}) + \sum_{i\in\mathcal{A}} H(\tilde{Z}_i | Z_\mathcal{V})\nonumber \\
&= H(Z_\mathcal{V}) - H(\tilde{Z}_\mathcal{A}) + \sum_{i\in\mathcal{A}} H(\epsilon_i)
\end{align}
using the chain rule for the joint entropy and the conditional independence of $\tilde{Z}_\mathcal{A}$ given $Z_\mathcal{V}$. 
Hence, we have 
\begin{equation}
MI(\mathcal{A}) = H(\tilde{Z}_\mathcal{A}) - \sum_{i\in \mathcal{A}} H(\epsilon_i)
\label{eq:simplified_MI}
\end{equation}
and a greater $MI(\cdot)$ indicates better prediction performance. 

The marginal MI of an additional noisy sample $\tilde{Z}_y$ given $\tilde{Z}_\mathcal{A}$, denoted as $MI(y|\mathcal{A})$ is given by
\begin{align}
MI(y|\mathcal{A}) &= MI(\mathcal{A}\cup\{y\}) - MI(\mathcal{A}) \nonumber \\
&= H(\tilde{Z}_\mathcal{A} \cup \tilde{Z}_y) - H(\tilde{Z}_\mathcal{A}) - H(\epsilon_y) \nonumber \\
&= H(\tilde{Z}_y|\tilde{Z}_\mathcal{A}) - H(\epsilon_y) \nonumber \\
&= H(Z_y|\tilde{Z}_\mathcal{A}) = \frac{1}{2}\log(2\pi e \sigma^2_{y|\tilde{A}}) \label{eq:marginal_MI}
\end{align}

\hl{Issue: in the current setting, $MI(\mathcal{A})$ is obviously submodular, but may not be monotonically non-decreasing.   
Given $\mathcal{K}(x,y)= 1 - ||x-y||/4$, $\sigma^2_0 = \max_{\epsilon_i} \sigma^2_{\epsilon_i}$, $|\mathcal{S}|=m$ and any two points in $\mathcal{S}$ have a pair-wise distance of at least $d$, can I come up with conditions (probably on $|\mathcal{A}|$) under which Eq.~\ref{eq:marginal_MI} is positive, namely, $\sigma^2_{y | \tilde{A}}\geq 1/(2\pi e)$ for any $\mathcal{A}\subseteq \mathcal{S}$ and any $y\in \mathcal{S}\setminus \mathcal{A}$?}

\subsection{Platform's Valuation Model}
To translate MI of selected sample locations $\mathcal{A}$ to (monetary) values that are comparable to costs and payments, the platform needs a valuation function $v: 2^\mathcal{S} \mapsto \mathbb{R}$, which is given by
\begin{equation}
v(\mathcal{A}) = c \cdot \log(1 + MI(\mathcal{A}))
\end{equation}
where the log function captures the diminishing returns behaviors in $MI(\cdot)$, and $c\geq 0$ is a known constant defined by the platform. 
Note that $v(\mathcal{A})$ is normalized, that is, $v(\emptyset)=0$. 

There exists interesting structural properties such as \textit{submodularity} and \textit{monotonicity} in $v(\cdot)$, which are very useful in later mechanism designs. 
Formally, given a finite set $\mathcal{C}$, a set function $f: 2^\mathcal{C} \mapsto \mathcal{R}$ is called \textit{submodular}, if $f(\mathcal{A} \cup \{x\}) - f(\mathcal{A}) \geq f(\mathcal{B} \cup \{x\}) - f(\mathcal{B})$ for any $\mathcal{A} \subseteq \mathcal{B} \subseteq \mathcal{C}$ and any $x \in \mathcal{C} \setminus \mathcal{B}$.
The notion of submodularity describes the diminishing returns behavior: adding a new element increases $f$ more, if there are fewer elements so far, and less, if there are more elements.
A set function $f: 2^\mathcal{C} \mapsto \mathcal{R}$ is said to be \textit{monotone} (non-decreasing), if $f(\mathcal{A}) \leq f(\mathcal{B})$ for any $\mathcal{A} \subseteq \mathcal{B} \subseteq \mathcal{C}$.

% \begin{mylemma}{}
% $MI(\mathcal{A})$ is submodular.
% \end{mylemma}
% \begin{proof}
% Since $H(\tilde{Z}_\mathcal{A})$ is well-known to be submodular and $\sum_{i\in \mathcal{A}} H(\epsilon_i)$ is modular in $\mathcal{A}$, $MI(\mathcal{A})$ in Eq.~\ref{eq:simplified_MI} is a submodular function in $\mathcal{A}$.
% \end{proof}
 
% If the valuation function $g(\cdot)$ over MI is nondecreasing concave, the valuation function $v(\mathcal{A}) = g(MI(\mathcal{A}))$ is also nondecreasing submodular.  

% \begin{mytheorem}
% If $g(\cdot)$ is nondecreasing concave, the valuation function $v(\mathcal{A}) = g(MI(\mathcal{A}))$ is nondecreasing submodular.
% \end{mytheorem}
% \begin{proof}
% Consider $\mathcal{A}\subseteq\mathcal{B}\subseteq\mathcal{S}$ and $y\in \mathcal{S}\setminus \mathcal{B}$. 
% Let $a=MI(\mathcal{A})$, $b=MI(\mathcal{A}\cup\{y\})$, $c=MI(\mathcal{B})$ and $d=MI(\mathcal{B}\cup\{y\})$.
% We have $b\geq a$, $d \geq c$, $a \leq c$, $b\leq d$ from monotonicity of $MI(\mathcal{A})$, and $b-a\geq d-c$ from submodularity of $MI(\mathcal{A})$.
% Define $b' = b+c-d\geq a$. 
% Then we have $g(b)-g(a)\geq g(b)-g(b')$ since $g(\cdot)$ is nondecreasing, and $g(b)-g(b')\geq g(d)-g(c)$, since $b-b'=d-c$, $b\leq d$ and $g(\cdot)$ is concave. 
% Hence, $g(b)-g(a) \geq g(d) - g(c)$ implies $v(\mathcal{A}\cup\{y\})-v(\mathcal{A}) \geq v(\mathcal{B}\cup\{y\})-v(\mathcal{B})$, which proves the submodularity of $v(\mathcal{A})$.

% Since $MI(\mathcal{A}\cup\{y\})\geq MI(\mathcal{A})$ and $g(\cdot)$ is nondecreasing, we have $g(MI(\mathcal{A}\cup\{y\}))\geq g(MI(\mathcal{A}))$, i.e., $v(\mathcal{A})$ is nondecreasing. 
% Hence, $v(\mathcal{A})$ is submodular and nondecreasing.
% \end{proof}

% If $v(\emptyset)=0$ (normalized), $v(\mathcal{A})$ is also non-negative.
% It is well-known that for a submodular, monotone and non-negative function like $MI(\mathcal{A})$ or $v(\mathcal{A})$, a greedy algorithm finds an approximate solution for $\max_{\mathcal{A}\subseteq \mathcal{S}, |\mathcal{A}|\leq k} MI(\mathcal{A}) \text{ or } v(\mathcal{A})$ within $1-1/e$ of the optimal solution, and no polynomial-time algorithm can achieve a better bound unless P = NP \cite{nemhauser1978analysis}.






==> sections/archive/system_models.tex <==
\section{System Model}
Fig.~\ref{fig:system_arch} illustrates our system, which consists of a centralized server called \textit{platform}, and spatially distributed mobile \textit{users} with sensing capability.
Each user knows its current location, whose device is registered and authenticated with the platform. 

As shown in the two-user example (Section~\ref{sec:example}), the platform's knowledge about users' sensing costs impacts the choice of incentive mechanisms. 
To this end, we consider two mechanisms, namely, \textit{pricing} and \textit{auction-based} mechanisms, as shown in Fig.~\ref{fig:arch_pricing} and \ref{fig:arch_auction}, respectively. 
The former assumes the knowledge of sensing cost distributions, which also takes care of the known-sensing-cost scenario by treating them as known deterministic cost distributions, but the later does not. 

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{1\columnwidth}
    \centering
    \includegraphics[width = 1\columnwidth]{./figs/arch_pricing}
    \caption{Pricing mechanism}
    \label{fig:arch_pricing}
    \end{subfigure}
    \begin{subfigure}[b]{1\columnwidth}
    \centering
    \includegraphics[width = 1\columnwidth]{./figs/arch_auction}
    \caption{Auction-based mechanism}
    \label{fig:arch_auction}
    \end{subfigure}
    \caption{System architecture for crowdsourced REM with (a) pricing and (b) auction-based mechanisms.}
    \label{fig:system_arch}
\end{figure}

In both mechanisms, the platform seeks to acquire sensing data from users periodically for the spectrum band of interest. 
In each period, the platform first announces a sensing task with detailed instructions (Step 1), such as desired center frequency, sampling rate, FFT parameters.
Assume that there are a set $\mathcal{S}=\{1,2,...,n\}$ of mobile users at locations $\{x_1, x_2, ..., x_n\}$ in the AoI, who are interested in participation after reading the task description.
Then they start interacting with the platform differently in the two mechanisms as described below.

\subsection{Pricing Mechanism}
In this mechanism, each user $i$ incurs a cost $C_i > 0$ for sensing ($C_i=0$ for not sensing), which is modeled as a random variable. 
Users then submit its current location and device type (Step 2), based on which the platform can estimate hardware noise and determine sampling values from the spatial model.
Besides, we assume that the platform can estimate cost distributions $\{f_{C_i}(c_i)\}$ from device types. 
In reality, it is very likely that data quality of a device is positively related to its hardware cost and thus sensing cost, that is, one sample from a more advanced device is more expensive but less noisy.

In Step 3, the platform sends leave-it-or-take-it offers ${\bf p}=[p_1,p_2, ..., p_m]^T$ to a set of users $\mathcal{A}\subseteq\mathcal{S}$, where $m=|\mathcal{A}|$.
Since each user $i\in \mathcal{A}$ only accepts it when $C_i\leq p_i$ with a probability of $F_{C_i}(p_i)$, only a subset of users $\mathcal{B}\subseteq\mathcal{A}$ will be recruited.
The platform aims to maximize the EU, 
\begin{equation}
\max_{\mathcal{A}\subseteq\mathcal{S}, {\bf p}} EU(\mathcal{A}, {\bf p}) = \max_{\mathcal{A}, {\bf p}}\sum_{\mathcal{B}\subseteq\mathcal{A}} u(\mathcal{B},{\bf p}) \cdot \text{Pr}(\mathcal{B}, {\bf p})
\end{equation}
where $u(\mathcal{B},{\bf p})=v(\mathcal{B})-\sum_{i\in\mathcal{B}} p_i$ is the achieved utility over $\mathcal{B}$ and $\text{Pr}(\mathcal{B}, {\bf p}) = \Pi_{i\in \mathcal{B}}F_{C_i}(p_i) \cdot \Pi_{j\in\mathcal{A}\setminus\mathcal{B}}F_{C_j}(p_j)$ is the corresponding probability.

Alternatively, the platform can maximize the ESV while keeping the expected total payment within the budget $B$,
\begin{align}
\max_{\mathcal{A}\subseteq\mathcal{S}, {\bf p}} & \sum_{\mathcal{B}\subseteq\mathcal{A}} v(\mathcal{B}) \cdot \text{Pr}(\mathcal{B}, {\bf p})\\
\text{Subject to } & \sum_{i\in \mathcal{A}} p_i \cdot F_{C_i}(p_i) \leq B
\end{align}
where $p_i \cdot F_{C_i}(p_i)$ is the expected payment to user $i\in \mathcal{A}$. 

Finally in Step 4, users make independent decisions and upload sensing data if they accept offers.
Note that Steps (3) and (4) may happen sequentially, that is, the platform makes offers one by one based on responses of previous offers. 


\subsection{Auction-Based Mechanism}
In this mechanism, each user $i$ submits a bid $b_i\geq c_i$, which is the reverse price for providing spectrum data, in addition to location and device type in Step 2.
The platform can again determine sampling values based on users' locations and hardware noise which is inferred from device types. 
Upon obtaining a bid-location-noise profile $({\bf b}, {\bf x}, \epsilon)$ where ${\bf b}=[b_1, b_2, ..., b_n]^T$, ${\bf x}=[x_1, x_2, ..., x_n]^T$ and $\epsilon=[\epsilon_1, \epsilon_2, ..., \epsilon_n]^T$, the platform executes a mechanism which selects a winner set $\mathcal{A}\subseteq\mathcal{S}$ and determines the payment $p_i \geq 0$ for each winner $i\in \mathcal{A}$. 
We assume that the mechanism has no positive transfer (i.e., $p_i=0$ for $i \notin \mathcal{A}$).
In Step 3, the platform notifies and pays winners, and obtains sensing data from them in Step 4. 

Since users are selfish, they may bid strategically on their costs and would like to maximize their utilities (i.e., $p_i-c_i$ if selected and 0 otherwise).
The platform is interested in designing a mechanism with the following desirable properties:
\begin{itemize}
\item \textbf{Computational efficiency} (CE): selection and payment rules can be computed in polynomial time.
\item \textbf{Individual rationality} (IR): each participating user will have a non-negative utility, i.e., $p_i \geq b_i$ for $i\in A$.
\item \textbf{Truthfulness} (TF): it is a dominant strategy for users to report their true costs regardless of other users' bids.
\end{itemize}

Since each user $i\in \mathcal{S}$ is uniquely associated with $(b_i, x_i, \epsilon_i)$, we use $\mathcal{S}$ to denote the bid-location-noise profile. 
Denote a mechanism as $\mathcal{M}=(\chi, \psi)$, where $\chi: 2^\mathcal{S} \mapsto 2^\mathcal{S}$ is the selection rule and $\psi: 2^\mathcal{S}\mapsto \mathbb{R}^n_+ $ is the payment rule.
The objective of the platform is to maximize the utility,
\begin{equation}
\max_{(\chi, \psi)} v(\chi(\mathcal{S})) - {\bf 1}^T \psi(\mathcal{S})
\end{equation}
where $\mathbf{1}=[1,...,1]^T$ is the $n$-by-$1$ column vector.
Alternatively, it can maximize the sampling value under a budget $B$,
\begin{align}
\max_{(\chi, \psi)} &~v(\chi(\mathcal{S})) \\
\text{Subject to } & {\bf 1}^T \psi(\mathcal{S}) \leq B
\end{align}
where the budget constraint is often called \textbf{budget feasibility} (BF) in mechanism design, in addition to CE, IR and TF.

In both mechanisms, we assume no entry or other overhead costs, that is, a user does not incur a fee to bid nor does it pay to communicate with the platform.
Besides, we assume users are of low mobility (e.g., pedestrians) and the displacement between the registered location and the eventual measurement location is small. 
We also assume users are non-collaborative and honest in following the protocol (e.g., no cheating with location or device type). Considerations of security and privacy enhancement is left as future work.


==> sections/pricing_mechanism2.tex <==
\subsection{Budget Constrained Value Maximization (VM)}\label{sec:value_maximization}
In this section, we describe how various pricing strategies may be applied to budget constrained value maximization.

\subsubsection{Budgeted VM with GA Pricing (VM-GA)}
With GA pricing $p(\cdot)$ given in Eq.~\ref{eq:GA_pricing_func}, the platform aims to 
\begin{align}
\max_{\mathcal{A}\subseteq\mathcal{S}} ~v & (\mathcal{A}) \label{eq:budgeted_value_maxization_goal}\\
\text{Subject to } p& (\mathcal{A}) \leq B \label{eq:budgeted_value_maxization_budget_constraint}
\end{align}
Note that the budget constraint is essentially the knapsack constraint, which is a generalization of the cardinality constraint. 

Since $v(\cdot)$ is a monotone, submodular, non-negative and normalized function (Section~\ref{sec:valuation_model}), the above becomes the classic submodular maximization with a knapsack constraint, which has been intensively studied, including \cite{sviridenko2004note, Krause2005,lin2010multi}.
Greedy algorithms that provide $(1-1/e)$ approximation have been proposed in \cite{sviridenko2004note, Krause2005}, but are very computationally expensive and thus impractical (the complexity is $\mathcal{O}(n^5)$ in general). 
In this study, we are interested in the modified greedy algorithm proposed by Lin \textit{et al.} in \cite{lin2010multi} that yields a $(1-1/\sqrt{e})\approx 0.39$ approximation guarantee at the cost of $\mathcal{O}(n^2)$ in terms of the number of queries to $v(\cdot)$.

\begin{algorithm}
\caption{{\tt GS($\mathcal{S}, v, \gamma, B$)}}
\label{algo:greedy_selection}
\LinesNumbered
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

\Input{$\mathcal{S}$ -- set of users, $v$ -- valuation function, $\gamma$ -- desired acceptance probability, $B$--budget} 
\Output{$\mathcal{A}$ -- set of selected users}
Let $p_i=F^{-1}_{C_i}(\gamma)$, $p(\mathcal{C})=\sum_{i\in\mathcal{C}} p_i$\;
$\mathcal{A}\leftarrow \emptyset$, $\mathcal{U}\leftarrow \mathcal{S}$\;
\While{$\mathcal{U} \neq \emptyset$}{
    $i\leftarrow \arg\max_{j\in \mathcal{U}}\frac{v(\mathcal{A} \cup \{j\}) - v(\mathcal{A})}{p_j}$\;
    \If{$p(\mathcal{A}) + p_i \leq B$}{
        $\mathcal{A}\leftarrow \mathcal{A}\cup\{i\}$, $\mathcal{U}\leftarrow\mathcal{U}\setminus\{i\}$\;
    }
}
$i^*\leftarrow \arg\max_{i\in \mathcal{S}, p_i\leq B} v(\{i\})$\;
\If{$v(\{i^*\}) \geq v(\mathcal{A})$}{
    $\mathcal{A}\leftarrow \{i^*\}$\;
}

\Return($\mathcal{A}$)\;
\end{algorithm}

The greedy selection (GS) algorithm is described in Algorithm~\ref{algo:greedy_selection}.
Given the current set $\mathcal{A}$, it greedily selects the next best user $i$ that maximizes the normalized marginal value $\frac{v(i|\mathcal{A})}{p(\{i\})}$, and keeps doing so until the budget is exhausted (Lines 3-6).
Then it compares the obtained $\mathcal{A}$ against the optimal singleton (Lines 7-9) to avoid the extreme case: 
the optimal solution is a singleton with a large cost (but within the budget), which may be missed by the above greedy procedure, since its normalized marginal value is small.
This extreme case may lead unbounded performance. 
In radio mapping, fortunately, a singleton is very unlikely to perform better than multiple samples, and hence we may ignore the last comparison.
In our case, the overall complexity in terms of the number of queries to $MI(i|\mathcal{A})$ is $\mathcal{O}(n^3)$.

For GA pricing, the platform can simply call {\tt GS}($\mathcal{S}, v, 1, B$) to obtain an approximate solution $\mathcal{A}$, and 
\begin{equation}
v(\mathcal{A}) \geq (1-1/\sqrt{e}) v(\mathcal{A}^*)
\end{equation}

\subsubsection{Budgeted VM with PA Pricing (VM-PA)}
The PA pricing function $p_\gamma(\cdot)$ is given in Eq.~\ref{eq:PA_pricing_func}. 
Similar to EU, we may define the expected value (EV) as follows,
\begin{equation}
EV_{\gamma}(\mathcal{A}) = \mathbb{E}_{\bf Y}[v(\mathcal{A}_{\bf y})]=\sum_{\bf y} \text{Pr}_{\gamma}({\bf y}) v(\mathcal{A}_{\bf y})
\end{equation}
where $\text{Pr}_{\gamma}({\bf y})=\gamma^{|\mathcal{A}_{\bf y}|} (1-\gamma)^{|\mathcal{A}|-|\mathcal{A}_{\bf y}|}$.
The objective\footnote{
It is also possible to impose the budget constraint on the expected total payment, that is, $\mathbb{E}_{\bf Y}[p_\gamma(\mathcal{A}_{\bf y})]=\sum_{i\in\mathcal{A}}  \gamma \cdot F^{-1}_{C_i}(\gamma) \leq B$. If so, the equivalent budget constraint becomes $p_\gamma(\mathcal{A}) \leq \frac{B}{\gamma}$ for a given $\gamma$. In this study, we are interested in the hard budget constraint. 
} is
\begin{align}
\max_{\mathcal{A}\subseteq\mathcal{S}} ~EV_{\gamma} & (\mathcal{A}) \nonumber\\
\text{Subject to } p_\gamma & (\mathcal{A}) \leq B \label{eq:ESV_maximization_PA}
\end{align}

Denote by $EV_{\gamma}(\mathcal{A}|\mathcal{B})$ the marginal EV of $\mathcal{A}$ conditioned on the set of recruited users $\mathcal{B}$, which is given by
\begin{equation}
	EV_{\gamma}(\mathcal{A}|\mathcal{B}) = \mathbb{E}_{\bf Y}[v(\mathcal{A}_{\bf y}|\mathcal{B})]
\end{equation}

Note that $EV_{\gamma}(\mathcal{A})$ and $EV_{\gamma}(\mathcal{A}|\mathcal{B})$ are submodular in $\mathcal{A}$ since the class of submodular functions are closed under taking expectations, as well as monotone and non-negative.

\begin{algorithm}
\caption{{\tt VM\_PA\_Single\_Batch($\mathcal{S}, f,\Gamma, B$)}}
\label{algo:VM_PA_single_batch}
\LinesNumbered
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

\Input{$\mathcal{S}$ -- set of users, $f$ -- objective function (either $v(\cdot)$ or $\hat{EV}(\cdot)$), $\Gamma=[\gamma_1,...,\gamma_l]$ -- candidate $\gamma$ values where $\gamma_1 < \gamma_2 < ... < \gamma_l$, $B$ -- budget} 
\Output{$\mathcal{A}$ -- set of selected users, ${\bf p}$ -- prices, $\gamma^*$ -- optimal desired acceptance probability}

$\mathcal{A} \leftarrow \emptyset$, $\gamma^*\leftarrow 0$, ${\bf p}\leftarrow NULL$\;
\ForEach{$\gamma$ in $[\gamma_1,...,\gamma_l]$}{
    $\mathcal{B} \leftarrow$ {\tt GS}($\mathcal{S}, f, \gamma, B$)\;
    \If{$\hat{EV}_{\gamma}(\mathcal{B}) > \hat{EV}_{\gamma^*}(\mathcal{A})$}{
        $\mathcal{A} \leftarrow \mathcal{B}$, $\gamma^* \leftarrow \gamma$\;
    }
}
\ForEach{$i$ in $\mathcal{A}$}{${\bf p} \leftarrow [{\bf p}, F^{-1}_{C_i}(\gamma^*)]$}


\Return($\mathcal{A}$, ${\bf p}$, $\gamma^*$)\;
\end{algorithm}


\vspace{0.2cm}
\noindent \textbf{Single-Batch Offering}\\
\indent We know from Proposition~\ref{eq:proposition_1} that for any chosen $\gamma$, the expected value of $\mathcal{A}$ returned by {\tt GS} (assuming no one rejects) has a lower bound, that is,
\begin{equation}
EV_{\gamma}(\mathcal{A}) \geq \gamma \cdot v(\mathcal{A})
\end{equation}
which is expected to be tight when $\gamma$ is close to 1 (e.g., 0.95).
But when $\gamma$ is relatively small, the bound can be very loose. 
Similar to the UM case, the platform may have two options.
The first option is to assume no rejections and work with $v(\cdot)$ by calling {\tt GS($\mathcal{S}, v, \gamma, B$)}, hoping that it could lead to a reasonably good EV.
Alternatively, it can approximate EV via MC simulations (denoted as $\hat{EV}_{\gamma}$), which can be otherwise very difficult to evaluate analytically, and call {\tt GS($\mathcal{S}, \hat{EV}_{\gamma}, \gamma, B$)}.
For convenience, we name the above two schemes as GS-v and GS-EV, respectively. 
It is easy to see that GS-EV is potentially time-consuming, and the approximation accuracy depends on the number of MC iterations, which can be limited in practice.

Intuitively, a smaller $\gamma$ implies lower payments to users and a larger $\mathcal{A}$ returned by {\tt GS}. 
Hence, there is a good chance for the platform to get a greater $EV$ by optimizing over $\gamma$, as described in Algo.~\ref{algo:VM_PA_single_batch}.
The corresponding complexity is $\mathcal{O}(ln^3)$, where $l$ is the number of candidate $\gamma$ values.

\vspace{0.2cm}
\noindent \textbf{From Single-Batch to Multi-Batch Offering}\\
\indent Similar to the UM case, the platform may repeat the same single-batch offering process and keep sending out more offers in batches based on the observed responses of previous offers, until either the budget is exhausted or the next batch cannot bring non-trivial marginal EV, as described in Algo.~\ref{algo:greedy_selection}. 

\begin{algorithm}
\caption{{\tt VM\_PA\_Multi\_Batch($\mathcal{S}, f, \Gamma, B, \alpha$)}}
\label{algo:VM_PA_multi_batch}
\LinesNumbered
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

\Input{$\mathcal{S}$ -- set of users, $f$ -- objective function (either $(\cdot)$ or $\hat{EV}_{\gamma}(\cdot)$), $\Gamma=[\gamma_1,...,\gamma_l]$ -- candidate $\gamma$ values where $\gamma_1 < \gamma_2 < ... < \gamma_l$, $B$ -- budget, $\alpha$ -- threshold for minimum marginal EV} 
\Output{$\mathcal{A}$ -- set of selected users, ${\bf p}$ -- prices, ${\bf y}$ -- user decisions}
$\mathcal{A} \leftarrow \emptyset$, ${\bf p} \leftarrow NULL$, ${\bf y}\leftarrow NULL$\;
\While{$\mathcal{S}\neq \emptyset$}{
    \If{$B>0$}{
    	$(\mathcal{B}, {\bf p}_\mathcal{B}, \gamma^*)$ $~~~~~\leftarrow${\tt VM\_PA\_Single\_Batch}($\mathcal{S}, f(\cdot|\mathcal{A}_{\bf y}), \Gamma, B$)  $//~f(\cdot|\mathcal{A}_{\bf y})$ is either $v(\cdot|\mathcal{A}_{\bf y})$ or $\hat{EV}_{\gamma}(\cdot|\mathcal{A}_{\bf y})$\;
    }
    \lElse{\textbf{break}}
    \If{ $\hat{EV}_{\gamma^*}(\mathcal{B}|\mathcal{A}_{\bf y}) > \alpha$ }{
        $B \leftarrow B - {\bf 1}^T {\bf p}_{\mathcal{B}}$, $\mathcal{S} \leftarrow \mathcal{S}\setminus \mathcal{B}$\;
        Send out offers $(\mathcal{B}, {\bf p}_\mathcal{B})$ and observe response ${\bf y}_\mathcal{B}$\;
        $\mathcal{A} \leftarrow \mathcal{A}\cup\mathcal{B}$, ${\bf p}\leftarrow [{\bf p}, {\bf p}_\mathcal{B}]$, ${\bf y}\leftarrow[{\bf y}, {\bf y}_\mathcal{B}]$\;
    }
    \lElse{\textbf{break}}
}

\Return($\mathcal{A}$, ${\bf p}$, ${\bf y}$)\;
\end{algorithm}

Note that in VM, the sequential offering is not as interesting as that in UM: the marginal EV of the next offer conditioned on currently recruited users is maximized when $\gamma=1$ (i.e., GA pricing), which means the platform cannot optimize $\gamma$ for each next offer (i.e., no OP pricing) and have to stick with a preset $\gamma$ instead.
Hence, we are mainly interested in PA pricing with single-batch or multi-batch offering for VM.



